Control of Humanoid Robots with Parallel Mechanisms using Differential Actuation Models

Several recently released humanoid robots, inspired by the mechanical design of Cassie, employ actuator configurations in which the motors are displaced from the joints to reduce leg inertia. While studies accounting for the full kinematic complexity have demonstrated the benefits of these designs, the associated loop-closure constraints greatly increase computational cost and limit their use in control and learning. As a result, the non-linear transmission is often approximated by a constant reduction ratio, preventing exploitation of the mechanism's full capabilities. This paper introduces a compact analytical formulation for the two standard knee and ankle mechanisms that captures the exact non-linear transmission while remaining computationally efficient. The model is fully differentiable up to second order with a minimal formulation, enabling low-cost evaluation of dynamic derivatives for trajectory optimization and of the apparent transmission impedance for reinforcement learning. We integrate this formulation into trajectory optimization and locomotion policy learning, and compare it against simplified constant-ratio approaches. Hardware experiments demonstrate improved accuracy and robustness, showing that the proposed method provides a practical means to incorporate parallel actuation into modern control algorithms.

==> tex/1.3.Introduction.tex <==
\section{Introduction}
Recent advances in biped locomotion have largely been driven by new hardware designs.
Many companies and research groups, designing the most recent biped robots, shifted toward serial-parallel architecture (see Fig.~\ref{Recent humanoids using parallel architectures}), especially in the leg design.
These architectures reduce limb reflected inertia and improve impact absorption \cite{batto_comparative_2023, mronga_whole-body_2022}, thereby enabling more dynamic movements, albeit at the cost of more complex modeling and control. 

\begin{figure}[!t]
\centering
\includegraphics[width=1\linewidth]{img/mosaic_legend.jpg}
\caption{Recent humanoids using parallel architectures. From top-left to bottom-right: Adam, A2, Atlas, T1, Digit V2, GR1, G1, H1, Walker S1 (Non exhaustive list)}
\label{Recent humanoids using parallel architectures}
\end{figure}

In most control frameworks - whether based on Whole-Body Model Predictive Control (WB-MPC) or Reinforcement Learning (RL) - motions are usually computed in the joint space using a serial dynamical model. 
Previous work \cite{kumar_model_2019} has shown that computation of the dynamics with a serial model of this type could decrease the computation time without leading to significant errors, especially when side-chain inertias are kept fixed in the robot model . A low level layer, provided by the robot manufacturer, is then in charge of converting controls from the joint space to the actuator space at control time \cite{eser_design_2021}.  
To mitigate the need for this conversion layer, some robot design rely on linear transmissions \cite{maslennikov_robust_2025, liao_berkeley_2024}.
Previous works focused on a tighter modeling of the parallel mechanism itself, through analytical approaches \cite{zhou_comprehensive_2018, kumar_analytical_2019, hoffman_modeling_2024}. Others addressed motion generation using either reduced-dimensional (but non-serial) models \cite{liang_reduced-dimensional_2025} or full-dimensional models \cite{matteis_optimal_2024, mronga_whole-body_2022, sovukluk_whole_2023, boukheddimi_investigations_2023}.
However, these last methods suffer from higher dimensionality and higher amount of constraints, leading to increased computational burden, making it difficult to run on real hardware. 

In RL, accounting for the full robot dynamics requires a simulator that supports closed-loop mechanisms. 
Until recently, such simulators were limited to CPU, making it challenging for locomotion policy learning \cite{li_reinforcement_2024}. 
Recent works used new generation GPU simulators such as Isaac Lab and Mujoco MJX to train locomotion policies with the full robot dynamics \cite{maslennikov_robust_2025, tanaka_mechanical_2025, amadio_learning_2025}. 
Despite some significant overhead, the computation time is only increased offline and does not impact policy inference.
However, these simulators rely on soft or approximate contacts models \cite{lidec_contact_2024} for constraining the closed chain, eventually increasing the sim to real gap and limiting deployments on real hardware.
This requires using specific techniques such as adversarial training, contact solver tuning, and observation space tuning to mitigate the drawbacks of the simulator \cite{maslennikov_robust_2025, tanaka_mechanical_2025, amadio_learning_2025}.

As a result, serial models remain the most practical choice for deploying locomotion policies on real robots.
While a recent study has shown that policy training with a serial model and an actuator-space output is possible \cite{zhang_lips_2025}, most of the recent breakthrough in RL - such as those demonstrated on Unitree robots - still rely on a serial dynamics model with a joint-space policy output, using the robot description files provided by the manufacturer. 
To the best of our knowledge, the way the serial controls are transformed to actuator controls for RL policies is not documented in the literature, and is kept closed source by robot manufacturers. 
Addressing this issue is one of the goals of this paper.

In the following,
\begin{itemize}

\item We first derive a \textbf{differential analytical models} of the geometric and kinematic mappings of the closed-loop transmissions composing modern robot architectures (Sec.~\ref{sec:actuation_model}).
\item We then propose a \textbf{Trajectory Optimization (TO)} algorithm that leverages this differential actuation model to generate motions with serial dynamics that would otherwise be infeasible, especially under actuator constraints. We also provide all the necessary components to extend this framework to WB-MPC (Sec. \ref{subsec:OCP_description}).  
\item We demonstrate an \textbf{series-parallel impedance transfer framework}  that uses the differential actuation model to transfer joint impedance from serial-space to actuator-space. This allows controlling robot with non-linear actuation using a RL policy trained in serial space (Sec. \ref{subsec:gains} and Sec. \ref{rldeploy}).  
\end{itemize}
% We first validate the effectiveness of our models in TO and then propose a RL framework along with a validation on a real biped robot.

% This paper will be structured as follows:
% First, in Sec.~\ref{sec:actuation_model}, we present a unified derivation of the geometric and kinematic mapping (so called Actuation models) for the knee and ankle mechanism and we compute their derivatives for their efficient use in both TO and RL, through impedance transfer.
% In Sec.~\ref{sec:implementation}, we then explain how we applied this method for TO (and how it can be extended to MPC) and for RL.
Finally, in Sec.~\ref{sec:results}, we analyze the results of our implementations, demonstrating the benefits of such approach in TO and its capabilities through an RL framework with impedance transfer. We also validate the method on a real robot with parallel actuation on both the knees and the ankles.

